Robust, privacy-preserving, transparent, and auditable on-device blocklisting

With the accelerated adoption of end-to-end encryption, there is an opportunity to re-architect security and anti-abuse primitives in a manner that preserves new privacy expectations. In this paper, we consider two novel protocols for on-device blocklisting that allow a client to determine whether an object (e.g., URL, document, image, etc.) is harmful based on threat information possessed by a so-called remote enforcer in a way that is both privacy-preserving and trustworthy. Our protocols leverage a unique combination of private set intersection to promote privacy, cryptographic hashes to ensure resilience to false positives, cryptographic signatures to improve transparency, and Merkle inclusion proofs to ensure consistency and auditability. We benchmark our protocols -- one that is time-efficient, and the other space-efficient -- to demonstrate their practical use for applications such as email, messaging, storage, and other applications. We also highlight remaining challenges, such as privacy and censorship tensions that exist with logging or reporting. We consider our work to be a critical first step towards enabling complex, multi-stakeholder discussions on how best to provide on-device protections.

==> Makefile <==
all: main.pdf

main.pdf:  *.tex
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main
	pdflatex main

clean:
	rm -f *.bak
	rm -f *~
	rm -f main.pdf
	rm -f main.ps
	rm -f *.log
	rm -f *.aux*
	rm -f *.dvi
	rm -f *.bbl
	rm -f *.blg
	rm -f *.idx
	rm -f *.out

rubber:
	rubber --pdf -Wall --warn misc main.tex
	rubber-info main.tex

watch:
	make rubber
	- while true; do \
	  	inotifywait -r -e DELETE_SELF -e MOVE_SELF -e MODIFY *.tex *.bib tables/*.tex figs/*; \
			make rubber; \
			sleep 1; \
		done

